GeneraLight: Improving Environment Generalization of Traffic Signal Control via Meta Reinforcement Learning

The heavy traffic congestion problem has always been a concern for modern cities. To alleviate traffic congestion, researchers use reinforcement learning (RL) to develop better traffic signal control (TSC) algorithms in recent years. However, most RL models are trained and tested in the same traffic flow environment, which results in a serious overfitting problem. Since the traffic flow environment in the real world keeps varying, these models can hardly be applied due to the lack of generalization ability. Besides, the limited number of accessible traffic flow data brings extra difficulty in testing the generalization ability of the models. In this paper, we design a novel traffic flow generator based on Wasserstein generative adversarial network to generate sufficient diverse and quality traffic flows and use them to build proper training and testing environments. Then we propose a meta-RL TSC framework GeneraLight to improve the generalization ability of TSC models. GeneraLight boosts the generalization performance by combining the idea of flow clustering and model-agnostic meta-learning. We conduct extensive experiments on multiple real-world datasets to show the superior performance of GeneraLight on generalizing to different traffic flows.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> apendix.tex <==
\newpage
\appendix

\section{Meta-testing Process of \our}

Algorithm \ref{alg:test} shows the meta-testing process of \our.

\begin{algorithm}[htbp]
\DontPrintSemicolon
\caption{Meta-testing Process of \our}
\label{alg:test}
\SetKwInOut{Input}{\textbf{Input}}\SetKwInOut{Output}{\textbf{Output}}
\KwIn{Traffic flow Distribution $D_{d}$ for testing; step size $\alpha$; Set of learned initialization $\left\{ \theta_{0}^{j} \right\}$ and $\theta_{p}$; total simulate time $T$; learning start time $T_{s}$}
\BlankLine
Sample traffic flows $\mathbf V_{i} \sim D_{d}$ \\
Empty feature collector $S, A, R$ \\
\For{\textbf{all} $\mathbf V_{i}$}
{
    \For{t $\longleftarrow$ 0, 1, 2, \dots, $T_{s} $, \dots, $T$}
    {
        \If{t < $T_{s}$}
        {
            Randomly choose action \\
            Collect state, action and reward to feature collector $S_{i}, A_{i}, R_{i}$\\
        }
        \If{t == $T_{s}$}
        {
            By cluster predictor, tailor $\mathbf V_{i}$ to cluster center $j \leftarrow f_{\theta_{p}}(<S_{i}, A_{i}, R_{i}>)$ \\
            Update parameter initialization $\theta_{i} \leftarrow \theta^{j}_{0}$
        }
        \If{t > $T_{s}$}
        {
            Generate and store transactions in $\mathcal M_{i}$ using $f_{\theta_{i}}$\\
            Update $\theta_{i} \leftarrow \theta_{i} - \alpha \nabla_{\theta}\mathcal L(f_{\theta}; \mathcal M_{i}) $ \\
        }
    }
}
\end{algorithm}

==> related_work_copy.tex <==
\section{Related Work}
\minisection{Reinforcement Learning for Traffic Signal Control}
Traffic signal control is an important topic in the transportation field for decades, which aims to optimize people's travel time by rescheduling the traffic signal plans. People in transportation fields have proposed many methods that highly rely on prior human knowledge~\cite{roess2004traffic, fellendorf1994vissim, mirchandani2001real, hunt1982scoot, lowrie1990scats, miller1963settings}. In recent years, using reinforcement learning to control the traffic signal has become a popular topic in both academia and industry~\cite{mannion2016experimental, wiering2000multi}. Learning-based traffic signal control method is more general in application since it does not require any manually predefined signal plan. Earlier learning-based works mainly utilize the idea of tabular Q-learning with discrete state representations~\cite{abdulhai2003reinforcement, el2010agent}, which is very limited when applied to large scale datasets.

Since the idea of deep reinforcement learning was proposed, people start to apply deep reinforcement learning methods to the traffic signal control problem. IntelliLight~\cite{wei2018intellilight} uses DQN~\cite{Mnih2015HumanlevelCT} algorithm to solve traffic signal control problem, by using many innovative designs for the representations of state and reward. Most of their designs are also adopted in following papers. FRAP~\cite{zheng2019learning} focuses on improve model performance by reducing the explore space, which makes it the state-of-the-art method in the single intersection environment. CoLight~\cite{wei2019colight} proposes to use the multi-head attention~\cite{velivckovic2017graph} to coordinate the traffic signals in multi-intersection environment, and use the parameter sharing mechanism to train multiple agents corresponding to each intersection. CoLight has achieved good results on several large-scale road networks. Since reinforcement learning algorithms generally take a long time to train, DemoLight~\cite{xiong2019learning} proposes to let reinforcement learning agents learn from some simple models, such as SOTL~\cite{cools2013self}, to speed up the training process. PressLight~\cite{wei2019presslight} redesigns the representation of state and reward, and get good performance in both single and multiple intersection environments. MPLight~\cite{chachatoward} combines the idea of FRAP and PressLight, and successfully conducted experiments on the super-large road network of 2510 intersections in Manhattan for the first time.

However, aforementioned RL methods have one common problem that they did not consider the generalization in different traffic environments. In most papers, they will train their agents for many rounds in an unchanged environment and test their agents in the same environment. MetaLight~\cite{Zang2020MetaLightVM} is the only exception which aims to train and test one agent for different intersections, such as train one agent on a four-way intersection and test it on a five-way intersection. MetaLight mainly focuses on the difference of action and observation spaces between training and testing phase. In this paper, we aim to design a traffic signal control model that can be generalized to different traffic environments, especially different traffic vehicle flows.

\minisection{Meta Reinforcement Learning} Meta reinforcement learning aims to solve a new reinforcement learning~\cite{Sutton1998ReinforcementLA} environment by utilizing the experience learned from a set of environments. The first approach is to use a recurrent network to learn from the experience in the training environments, such as RL2~\cite{Duan2016RL2FR} and \cite{Wang2017LearningTR}. Then, people begin to solve this problem in different ways: SNAIL~\cite{Mishra2018ASN} combines the idea of wavenet~\cite{Oord2016WaveNetAG} and RL2 to better utilize historical information; EPG~\cite{Houthooft2018EvolvedPG} uses a meta loss function to store the information of different environments, and update the loss function by evolution algorithm~\cite{Banzhaf1998GeneticP}. MetaGenRL~\cite{Kirsch2019ImprovingGI} improves EPG by redesign the meta loss function which can be optimized by gradient descent to save training time. MAESN~\cite{Gupta2018MetaReinforcementLO} adds noise as a part of the state, which can enhance the exploration ability of policy to adapt to different environments. Some methods utilize the idea of domain randomization~\cite{Tobin2017DomainRF, OpenAI2019SolvingRC}. With the help of evolution algorithm, POET~\cite{Wang2019PairedOT} can finish the learning process from simple to complex environments. Some people think robust optimization~\cite{Abdullah2019WassersteinRR, Kuhn2019WassersteinDR, Jafra2019RobustRL, Smirnova2019DistributionallyRR} is also a possible solution. EPOPT~\cite{Rajeswaran2017EPOptLR} searches the environment in train set to find some hard environments, and use the idea of CAaR~\cite{Rockafellar2000OPTIMIZATIONOC} to optimize policy on the hard environments. RARL~\cite{Pinto2017RobustAR} uses adversarial networks~\cite{Goodfellow2014GenerativeAN} to improve the robustness of model. People have recently proposed novel unsupervised learning-based models to solve this problem~\cite{Eysenbach2018DiversityIA, Gupta2018UnsupervisedMF}. As far as we know, there is currently no meta reinforcement learning method for multi-agent reinforcement learning.

MAML~\cite{Finn2017ModelAgnosticMF} is the most popular meta-learning algorithm that aims to optimize the global parameter initialization, which significantly
improves the effectiveness and efficiency of reinforcement learning on unseen environments. However, people find that only one global initialization is not enough for diverse environments: MUMOMAML~\cite{Vuorio2018TowardMM} uses environment-specific global initialization for different environments. HSML~\cite{Yao2019HierarchicallySM} aims to tailor the global initialization to each environment, by a hierarchical structure that combines the embedding of environments and global initialization. In this paper, we follow their tailor idea and proposed \our, which combines the idea of clustering~\cite{MacQueen1967SomeMF} to better tailor the global initialization to different environments.
